The SDSS-III Baryon Oscillation Spectroscopic Survey: The Quasar Luminosity Function from Data Release Nine

We present a new measurement of the optical Quasar Luminosity Function (QLF), using data from the Sloan Digital Sky Survey-III: Baryon Oscillation Spectroscopic Survey (SDSS-III: BOSS). From the SDSS-III Data Release Nine (DR9), we select a uniform sample of 22,301 i<=21.8 quasars over an area of 2236 sq. deg with confirmed spectroscopic redshifts between 2.2<z<3.5, filling in a key part of the luminosity-redshift plane for optical quasar studies. We derive the completeness of the survey through simulated quasar photometry, and check this completeness estimate using a sample of quasars selected by their photometric variability within the BOSS footprint. We investigate the level of systematics associated with our quasar sample using the simulations, in the process generating color-redshift relations and a new quasar k-correction. We probe the faint end of the QLF to M_i(z=2.2) = -24.5 and see a clear break in the QLF at all redshifts up to z=3.5. We find that a log-linear relation (in log[Phi*] - M*) for a luminosity and density evolution (LEDE) model adequately describes our data within the range 2.2<z<3.5; across this interval the break luminosity increases by a factor of ~2.3 while Phi* declines by a factor of ~6. At z<2.2 our data is reasonably well fit by a pure luminosity evolution (PLE) model. We see only a weak signature of "AGN downsizing", in line with recent studies of the hard X-ray luminosity function. We compare our measured QLF to a number of theoretical models and find that models making a variety of assumptions about quasar triggering and halo occupation can fit our data over a wide range of redshifts and luminosities.

==> README <==



	S D S S  - I I I 
	Baryon Oscillation Spectroscopic Survey (B O S S) 
	The Quasar Luminosity Function from Data Release Nine

AUTHORS:
Nicholas P. Ross (npross@lbl.gov), Ian D. McGreer, Martin White, Gordon T. Richards, Adam D. Myers, Nathalie Palanque-Delabrouille, Michael A. Strauss, Scott F. Anderson, Yue Shen, W. N. Brandt, Christophe Yeche, Molly E. C. Swanson et al., for the SDSS-III: BOSS Quasar Working Group. 


ABSTRACT:
We present a new measurement of the optical Quasar Luminosity Function
(QLF), using data from the Sloan Digital Sky Survey-III: Baryon
Oscillation Spectroscopic Survey (SDSS-III: BOSS).  From the SDSS-III
Data Release Nine (DR9), we select a uniform sample of \hbox{22,301}
$i\lesssim21.8$ quasars over an area of 2236~deg$^{2}$ with confirmed
spectroscopic redshifts between $2.2<z<3.5$, filling in a key part of
the luminosity-redshift plane for optical quasar studies.
We derive the completeness of the survey through simulated quasar
photometry, and check this completeness estimate using a sample of
quasars selected by their photometric variability within the BOSS
footprint. We investigate the level of systematics associated with
our quasar sample using the simulations, in the process generating
color-redshift relations and a new quasar $k$-correction.
We probe the faint end of the QLF to $M_{i}(z=2.2)\approx-24.5$ and
see a clear break in the QLF at all redshifts up to $z=3.5$. We find
that a log-linear relation (in $\log\Phi^{*}-M^{*}$) for a luminosity
and density evolution (LEDE) model adequately describes our data
within the range $2.2<z<3.5$; across this interval the break
luminosity increases by a factor of $\sim$2.3 while $\Phi^{*}$
declines by a factor of $\sim$6.  At $z\lesssim2.2$ our data is
reasonably well fit by a pure luminosity evolution (PLE) model.
We see only a weak signature of ``AGN downsizing'', in line with recent
studies of the hard X-ray luminosity function.
We compare our measured QLF to a number of theoretical models and find that
models making a variety of assumptions about quasar triggering and halo
occupation can fit our data over a wide range of redshifts and luminosities.


NOTES:



PAGE CHARGES:
Nicholas P. Ross 
David J. Schlegel. 
Lawrence Berkeley National Lab
1 Cyclotron Road 
MS 50R-5032
Berkeley, CA 94720, USA


CONTACT:
Nicholas P. Ross
npross@lbl.gov
Lawrence Berkeley National Lab
1 Cyclotron Road 
MS 50R-5032
Berkeley, CA 94720, USA
Tel: 510-495-2595


LAST UPDATED:
Mon Oct 22 17:45:26 PDT 2012

